Survey on Combinatorial Register Allocation and Instruction Scheduling

Register allocation (mapping variables to processor registers or memory) and instruction scheduling (reordering instructions to increase instruction-level parallelism) are essential tasks for generating efficient assembly code in a compiler. In the last three decades, combinatorial optimization has emerged as an alternative to traditional, heuristic algorithms for these two tasks. Combinatorial optimization approaches can deliver optimal solutions according to a model, can precisely capture trade-offs between conflicting decisions, and are more flexible at the expense of increased compilation time. This paper provides an exhaustive literature review and a classification of combinatorial optimization approaches to register allocation and instruction scheduling, with a focus on the techniques that are most applied in this context: integer programming, constraint programming, partitioned Boolean quadratic programming, and enumeration. Researchers in compilers and combinatorial optimization can benefit from identifying developments, trends, and challenges in the area; compiler practitioners may discern opportunities and grasp the potential benefit of applying combinatorial optimization.

==> figures/styles.tex <==
\definecolor{tempcolor1}{rgb}{0.85,0.85,0.85}%
\definecolor{tempcolor2}{rgb}{0.65,0.65,0.65}%
\definecolor{tempcolor3}{rgb}{0.95,0.95,0.95}%
\definecolor{tempcolor4}{rgb}{0.75,0.75,0.75}%
\definecolor{tempcolor5}{rgb}{0.55,0.55,0.55}%
\colorlet{background}{black!35}
\newdimen\zerolinewidth%
\newdimen\cornerRadius%
\cornerRadius=3pt%
\tikzset{%
  zero line width/.code={%
    \zerolinewidth=\pgflinewidth
    \tikzset{line width=0cm}%
  },
  use line width/.code={%
    \tikzset{line width=\the\zerolinewidth}%
  },
  structure/.style={%
    text=structure,
  },
  draw structure/.style={%
    draw=structure,
  },
  fill structure/.style={%
    fill=structure,
  },
  alt/.code args={<#1>#2#3}{%
    \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}},
  },
  fill structure on/.style={alt=#1{fill structure}{}},
  draw structure on/.style={alt=#1{draw structure}{}},
  structure on/.style={alt=#1{structure}{}},
  file/.style={%
    inner sep=0.2cm,
    outer sep=0,
    node distance=1cm,
  },
  unison file/.style={%
    file,
    text=structure
  },
  input/.style={%
    file,
  },
  output/.style={%
    file,
  },
  connection node/.style={%
    circle,
    draw,
    line width=1mm,
    minimum width=1.5cm,
  },
  box/.style={%
    draw,
    line width=0.2mm,
    fill=white,
  },
  problem/.style={%
    box,
    rounded corners=\cornerRadius,
    inner xsep=0.5mm,
  },
  problem scope/.style={%
    box,
    dashed,
    inner xsep=2mm,
    inner ysep=5mm,
    rounded corners=\cornerRadius,
    yshift=-4mm,
  },
  problem scope label/.style={
    font=\small,
    yshift=-10.5mm,
  },
  block/.style={%
    box,
    rounded corners=\cornerRadius,
  },
  cfg block/.style={%
    block,
    minimum width=4.2cm,
  },
  sum cfg block/.style={%
    block,
    minimum width=5.6cm,
  },
  mini cfg block/.style={%
    block,
    minimum width=1.5cm,
    minimum height=1cm,
    node distance=0.4cm,
  },
  mini cfg code/.style={%
    below right,
    xshift=-0.35cm
  },
  single instruction/.style={%
    yshift=-0.25cm
  },
  big cfg block/.style={%
    block,
    minimum width=7cm,
  },
  block label/.style={%
  },
  block border/.style={%
    draw,
    line width=1mm,
  },
  block variables/.style={%
    fill=white,
  },
  stage/.style={%
    box,
    inner xsep=5mm,
    inner ysep=5mm,
    fill=unisonbg
  },
  solver step/.style={%
    node distance=0cm,
  },
  data/.style={%
    minimum width=5cm,
    minimum height=3cm,
    node distance=4cm,
  },
  congruences/.style={%
  },
  cover/.style={%
    box,
    dashed,
    line width=1mm,
    inner xsep=5mm,
    inner ysep=5mm,
  },
  flow/.style={%
    ->,
    >=stealth,
    line width=0.2mm,
  },
  secondary flow/.style={%
    ->,
    >=stealth,
    line width=1mm,
    dash pattern=on 3mm off 3mm,
  },
  connection edge/.style={%
    line width=1mm,
  },
  must connect/.style={%
    connection edge,
  },
  may connect/.style={%
    connection edge,
    loosely dashed
  },
  unison/.style={%
    inner xsep=20mm,
    inner ysep=10mm,
  },
  unison stage/.style={%
    box,
    minimum width=4.5cm,
    minimum height=2.2cm,
    node distance=2.7cm,
    fill=unisonbg
  },
  external stage/.style={%
    unison stage,
    fill=white
  },
  unison data/.style={%
    box,
    rounded corners=\cornerRadius,
    minimum width=4.5cm,
    minimum height=2.2cm,
    node distance=2.7cm
  },
  zoom/.style={%
    line width=1mm,
    dash pattern=on 3mm off 3mm,
  },
  focus/.style={%
    draw,
    line width=0.5mm,
    dash pattern=on 3mm off 3mm,
    inner sep=5mm,
  },
  minsizeblock/.style={%
    block,
    minimum width=3cm,
    minimum height=3cm
  },
  square/.style={%
    fill=white,
    minimum size=13mm,
    inner sep=0,
    outer sep=0,
    node distance=0,
  },
  thin liveness/.style={%
    draw,
    line width=0.7mm,
  },
  live range/.style={%
      <->,
      >=*,
      line width=0.1mm,
    },
  tree line/.style={%
    draw,
    line width=0.35mm,
  },
  statement/.style={%
    minimum size=0.15cm,
    inner sep=0pt,
    node distance=0.7cm,
  },
  program point/.style={%
    fill,
    circle,
    fill=black,
    minimum size=0.15cm,
    inner sep=0pt,
    node distance=0.7cm,
  },
  ora variable/.style={%
    font=\small,
  },
  triangle/.style = {draw, regular polygon, regular polygon sides=3 },
  pra/.style={%
    fill,
    fill=white,
    node distance=0.3cm,
  },
  pra source/.style={%
    pra,
    triangle,
    shape border rotate=180,
    minimum size=0.49cm,
    inner sep=0.0cm,
  },
  pra source right/.style={%
    pra source,
    shape border rotate=270,
  },
  pra sink/.style={%
    pra,
    triangle,
    minimum size=0.49cm,
    inner sep=0.0cm,
  },
  pra sink left/.style={%
    pra source,
    shape border rotate=90,
  },
  pra storage/.style={%
    pra,
    draw,
    circle,
    minimum size=0.49cm,
    inner sep=0.03cm,
  },
  pra fit/.style={%
    draw,
    draw=gray,
    node distance=0cm,
    inner sep=0.06cm,
    rounded corners=\cornerRadius,
  },
  pra bar/.style={%
    pra fit,
  },
  pra crossbar/.style={%
    pra fit,
    fill=gray!15,
  },
  pra dots/.style={%
    node distance=0.3cm,
  },
  pra label/.style={%
  },
}%
\pgfdeclarelayer{layer0}%
\pgfdeclarelayer{layer1}%
\pgfdeclarelayer{layer2}%
\pgfdeclarelayer{layer3}%
\pgfdeclarelayer{layer4}%
\pgfdeclarelayer{layer5}%

